Do LiDAR Language Models Really Understand Spatio-temporal Relationships?

Recent 4D LiDAR language models aim to reason about objects and their evolving spatial relationships. Yet, in our evaluation, always selecting the same option nearly matches the multiple-choice accuracy of two B4DL-derived configurations. We introduce LiDAR-Hallu, a geometry-referenced benchmark and diagnostic protocol with 10,000 questions across 150 nuScenes scenes. It covers object existence, ego-relative position, distance ordering, relative motion, and temporal localization, with explicit rules for selecting objects, comparing times, and determining reference answers. Our protocol combines fixed-answer and candidate-content controls, cross-scene pairs with identical prompts but opposite reference answers, and relation-specific recall. Analysis of 100,000 recorded responses reveals failures hidden by aggregate accuracy. Candidate duration alone makes temporal answers predictable without observing LiDAR. On paired questions, the models frequently give the same answer to scenes requiring opposite answers. Relation-specific analysis further shows that both configurations miss every positive lateral-motion case across all tested conditions. Temporal-shuffle contrastive decoding provides little net improvement, as repairs are largely offset by new errors and the main failures persist. These results show that evaluating spatio-temporal reasoning requires testing whether models distinguish the queried physical relationships, rather than relying on individual-answer accuracy alone. The source code, checkpoints, and data are released at https://github.com/Awesome4D/4DMLLM_Hallucination_Bench.

==> references_backup.tex <==
@inproceedings{caesar2020nuscenes,
 title={{nuScenes}: A Multimodal Dataset for Autonomous Driving},
 author={Caesar, Holger and Bankiti, Varun and Lang, Alex H. and Vora, Sourabh and Liong, Venice Erin and Xu, Qiang and Krishnan, Anush and Pan, Yu and Baldan, Giancarlo and Beijbom, Oscar},
 booktitle={Proc. IEEE/CVF CVPR},pages={11621--11631},year={2020}}
@article{hess2022lidarclip,
 title={{LidarCLIP} or: How I Learned to Talk to Point Clouds},
 author={Hess, Georg and Tonderski, Adam and Petersson, Christoffer and {\AA}str{\"o}m, Kalle and Svensson, Lennart},
 journal={arXiv preprint arXiv:2212.06858},year={2022}}
@inproceedings{yang2025lidar,
 title={{LiDAR-LLM}: Exploring the Potential of Large Language Models for {3D LiDAR} Understanding},
 author={Yang, Senqiao and Liu, Jiaming and Zhang, Ray and Pan, Mingjie and Guo, Zoey and Li, Xiaoqi and Chen, Zehui and Gao, Peng and Guo, Yandong and Zhang, Shanghang},
 booktitle={Proc. AAAI},volume={39},number={9},pages={9247--9255},year={2025}}
@inproceedings{choi2025b4dl,
 title={{B4DL}: A Benchmark for {4D LiDAR LLM} in Spatio-Temporal Understanding},
 author={Choi, Changho and Shin, Youngwoo and Han, Gyojin and Lee, Dong-Jae and Kim, Junmo},
 booktitle={Proc. ACM Multimedia},pages={3399--3407},year={2025}}
@inproceedings{qian2024nuscenesqa,
 title={{NuScenes-QA}: A Multi-Modal Visual Question Answering Benchmark for Autonomous Driving Scenario},
 author={Qian, Tianwen and Chen, Jingjing and Zhuo, Linhai and Jiao, Yang and Jiang, Yu-Gang},
 booktitle={Proc. AAAI},volume={38},number={5},pages={4542--4550},year={2024}}
@inproceedings{sima2024drivelm,
 title={{DriveLM}: Driving with Graph Visual Question Answering},
 author={Sima, Chonghao and Renz, Katrin and Chitta, Kashyap and Chen, Li and Zhang, Hanxue and Xie, Chengen and Bei{\ss}wenger, Jens and Luo, Ping and Geiger, Andreas and Li, Hongyang},
 booktitle={Proc. ECCV},year={2024}}
@article{tian2025spatialqa,
 title={{NuScenes-SpatialQA}: A Spatial Understanding and Reasoning Benchmark for Vision-Language Models in Autonomous Driving},
 author={Tian, Kexin and Mao, Jingrui and Zhang, Yunlong and Jiang, Jiwan and Zhou, Yang and Tu, Zhengzhong},
 journal={arXiv preprint arXiv:2504.03164},year={2025}}
@article{vo2026drivespatial,
 title={{DriveSpatial}: A Benchmark for Spatiotemporal Intelligence in {VLMs} for Autonomous Driving},
 author={Vo, Hao and Vo, Khoa and Nguyen, Phu Loc and Tran, Sieu and Nguyen, Duc Minh and Cuong, Ngo Xuan and Gawugah, Gladys and Godavarthi, Sreevenkata Anjani Tishita and Rainwater, Chase and Bui, Nghi D. Q. and Nguyen, Anh and Nguyen, Duy Minh Ho and Le, Ngan},
 journal={arXiv preprint arXiv:2605.23176},year={2026}}
@inproceedings{thrush2022winoground,
 title={Winoground: Probing Vision and Language Models for Visio-Linguistic Compositionality},
 author={Thrush, Tristan and Jiang, Ryan and Bartolo, Max and Singh, Amanpreet and Williams, Adina and Kiela, Douwe and Ross, Candace},
 booktitle={Proc. IEEE/CVF CVPR},pages={5238--5248},year={2022}}
@inproceedings{yuksekgonul2023aro,
 title={When and Why Vision-Language Models Behave like Bags-of-Words, and What to Do About It?},
 author={Yuksekgonul, Mert and Bianchi, Federico and Kalluri, Pratyusha and Jurafsky, Dan and Zou, James},
 booktitle={Proc. ICLR},year={2023}}
@inproceedings{rohrbach2018object,
 title={Object Hallucination in Image Captioning},
 author={Rohrbach, Anna and Hendricks, Lisa Anne and Burns, Kaylee and Darrell, Trevor and Saenko, Kate},
 booktitle={Proc. EMNLP},pages={4035--4045},year={2018}}
@inproceedings{li2023evaluating,
 title={Evaluating Object Hallucination in Large Vision-Language Models},
 author={Li, Yifan and Du, Yifan and Zhou, Kun and Wang, Jinpeng and Zhao, Wayne Xin and Wen, Ji-Rong},
 booktitle={Proc. EMNLP},pages={292--305},year={2023}}
@article{wang2023amber,
 title={{AMBER}: An {LLM}-free Multi-dimensional Benchmark for {MLLMs} Hallucination Evaluation},
 author={Wang, Junyang and Wang, Yuhang and Xu, Guohai and Zhang, Jing and Gu, Yukai and Jia, Haitao and Wang, Jiaqi and Xu, Haiyang and Yan, Ming and Zhang, Ji and others},
 journal={arXiv preprint arXiv:2311.07397},year={2023}}
@inproceedings{li2025vidhalluc,
 title={{VidHalluc}: Evaluating Temporal Hallucinations in Multimodal Large Language Models for Video Understanding},
 author={Li, Chaoyu and Im, Eun Woo and Fazli, Pooyan},
 booktitle={Proc. IEEE/CVF CVPR},pages={13723--13733},year={2025}}
@inproceedings{leng2024vcd,
 title={Mitigating Object Hallucinations in Large Vision-Language Models through Visual Contrastive Decoding},
 author={Leng, Sicong and Zhang, Hang and Chen, Guanzheng and Li, Xin and Lu, Shijian and Miao, Chunyan and Bing, Lidong},
 booktitle={Proc. IEEE/CVF CVPR},pages={13872--13882},year={2024}}
@inproceedings{pezeshkpour2024order,
 title={Large Language Models Sensitivity to The Order of Options in Multiple-Choice Questions},
 author={Pezeshkpour, Pouya and Hruschka, Estevam},
 booktitle={Findings of NAACL},pages={2006--2017},year={2024}}
@inproceedings{xue2024symbol,
 title={Strengthened Symbol Binding Makes Large Language Models Reliable Multiple-Choice Selectors},
 author={Xue, Mengge and Hu, Zhenyu and Liu, Liqun and Liao, Kuo and Li, Shuang and Han, Honglin and Zhao, Meng and Yin, Chengguo},
 booktitle={Proc. ACL},pages={4331--4344},year={2024}}
@article{zhu2025four,
 title={{4D-Bench}: Benchmarking Multi-modal Large Language Models for {4D} Object Understanding},
 author={Zhu, Wenxuan and Li, Bing and Zheng, Cheng and Mai, Jinjie and Chen, Jun and Jiang, Letian and Hamdi, Abdullah and Martinez, Sara Rojas and Lin, Chia-Wen and Elhoseiny, Mohamed and Ghanem, Bernard},
 journal={arXiv preprint arXiv:2503.17827},year={2025}}
@article{wang2026spatial,
 title={{Spatial4D-Bench}: A Versatile {4D} Spatial Intelligence Benchmark},
 author={Wang, Pan and Liu, Yang and Wu, Guile and others},
 journal={arXiv preprint arXiv:2601.00092},year={2026}}

@article{ma2026real3dqa,
 title={Do 3D Large Language Models Really Understand 3D Spatial Relationships?},
 author={Ma, Xianzheng and Sun, Tao and Chen, Shuai and Bhalgat, Yash and Gu, Jindong and Chang, Angel X. and Armeni, Iro and Laina, Iro and Peng, Songyou and Prisacariu, Victor Adrian},
 journal={arXiv preprint arXiv:2603.23523},year={2026}}

@article{zhang2024eventhallusion,
 title={{EventHallusion}: Diagnosing Event Hallucinations in Video {LLMs}},
 author={Zhang, Jiacheng and Jiao, Yang and Chen, Shaoxiang and Zhao, Na and Tan, Zhiyu and Li, Hao and Chen, Jingjing},
 journal={arXiv preprint arXiv:2409.16597},year={2024}}

@inproceedings{goyal2017making,
 title={Making the {V} in {VQA} Matter: Elevating the Role of Image Understanding in Visual Question Answering},
 author={Goyal, Yash and Khot, Tejas and Summers-Stay, Douglas and Batra, Dhruv and Parikh, Devi},
 booktitle={Proc. IEEE CVPR},year={2017}}

@inproceedings{agrawal2018priors,
 title={Don't Just Assume; Look and Answer: Overcoming Priors for Visual Question Answering},
 author={Agrawal, Aishwarya and Batra, Dhruv and Parikh, Devi and Kembhavi, Aniruddha},
 booktitle={Proc. IEEE CVPR},pages={4971--4980},year={2018}}

@article{huang2025beacon3d,
 title={Unveiling the Mist over {3D} Vision-Language Understanding: Object-centric Evaluation with Chain-of-Analysis},
 author={Huang, Jiangyong and Jia, Baoxiong and Wang, Yan and Zhu, Ziyu and Linghu, Xiongkun and Li, Qing and Zhu, Song-Chun and Huang, Siyuan},
 journal={arXiv preprint arXiv:2503.22420},year={2025}}

@inproceedings{marcu2024lingoqa,
 title={{LingoQA}: Visual Question Answering for Autonomous Driving},
 author={Marcu, Ana-Maria and Chen, Long and H{\"u}nermann, Jan and Karnsund, Alice and Hanotte, Benoit and Chidananda, Prajwal and Nair, Saurabh and Badrinarayanan, Vijay and Kendall, Alex and Shotton, Jamie and Arani, Elahe and Sinavski, Oleg},
 booktitle={Proc. ECCV},pages={252--269},year={2024}}

@article{xu2024drivegpt4,
 title={{DriveGPT4}: Interpretable End-to-End Autonomous Driving via Large Language Model},
 author={Xu, Zhenhua and Zhang, Yujia and Xie, Enze and Zhao, Zhen and Guo, Yong and Wong, Kwan-Yee K. and Li, Zhenguo and Zhao, Hengshuang},
 journal={IEEE Robotics and Automation Letters},volume={9},number={10},pages={8186--8193},year={2024}}

